Tuning and optimization for a variety of many-core architectures without changing a single line of implementation code using the Alpaka library

We present an analysis on optimizing performance of a single C++11 source code using the Alpaka hardware abstraction library. For this we use the general matrix multiplication (GEMM) algorithm in order to show that compilers can optimize Alpaka code effectively when tuning key parameters of the algorithm. We do not intend to rival existing, highly optimized DGEMM versions, but merely choose this example to prove that Alpaka allows for platform-specific tuning with a single source code. In addition we analyze the optimization potential available with vendor-specific compilers when confronted with the heavily templated abstractions of Alpaka. We specifically test the code for bleeding edge architectures such as Nvidia's Tesla P100, Intel's Knights Landing (KNL) and Haswell architecture as well as IBM's Power8 system. On some of these we are able to reach almost 50\% of the peak floating point operation performance using the aforementioned means. When adding compiler-specific #pragmas we are able to reach 5 TFLOPS/s on a P100 and over 1 TFLOPS/s on a KNL system.

==> content/power8_autotuning.tex <==
\begin{figure}[t]
\centering
\begin{minipage}{0.495\textwidth}
\centering
\textbf{Single precision, XL compiler}

\begin{tikzpicture}
	\begin{loglogaxis}[
		width=0.9\textwidth,
		height=0.27\textheight,
		major tick length={1.5pt},
		xlabel={Tile size $T$},
		xtick={16,32,64,128,256,512},
		xticklabels={16,32,64,128,256,512},
		xlabel style={font=\scriptsize},
		xticklabel style={font=\scriptsize},
		ylabel={Hardware threads per core},
		ytick={20,40,80,160},
		yticklabels={1,2,4,8},
		ylabel style={font=\scriptsize},
		yticklabel style={font=\scriptsize},
		zlabel={\GFLOPS},
		grid=major,
		xmin = 10,
		xmax = 850,
		ymin = 13,
		ymax = 250,
		major grid style={dotted},
		colorbar,
		colorbar/width=5pt,
		colormap name=mycolormap,
		colorbar style={ylabel={achieved \GFLOPS{}},yticklabel style={font=\tiny,text width=0.7em,}},
		view={0}{90},
	]

	\addplot3[ %
	    scatter=true,
	    only marks,
	    mark=*,
	    color=black,
	    point meta=explicit,
	    visualization depends on = {z/11 \as \perpointmarksize},
	    scatter/@pre marker code/.append style={/tikz/mark size=\perpointmarksize},
	    visualization depends on={meta \as \nodedescription},
	    nodes near coords*={\numprint{\nodedescription}},
		every node near coord/.append style={xshift=0pt,yshift=-16pt,font=\tiny},
	]  table[x=tilesize,y=core_count,z=power8_xl_float_size_10,meta=power8_xl_float_10] {./results/power8_autotuning.csv};
	\end{loglogaxis}
\end{tikzpicture}

\end{minipage}
\begin{minipage}{0.495\textwidth}
\centering
\textbf{Double precision, XL compiler}
\begin{tikzpicture}
	\begin{loglogaxis}[
		width=0.9\textwidth,
		height=0.27\textheight,
		major tick length={1.5pt},
		xlabel={Tile size $T$},
		xtick={16,32,64,128,256,512},
		xticklabels={16,32,64,128,256,512},
		xlabel style={font=\scriptsize},
		xticklabel style={font=\scriptsize},
		ylabel={Hardware threads per core},
		ytick={20,40,80,160},
		yticklabels={1,2,4,8},
		ylabel style={font=\scriptsize},
		yticklabel style={font=\scriptsize},
		zlabel={\GFLOPS},
		grid=major,
		xmin = 10,
		xmax = 850,
		ymin = 13,
		ymax = 250,
		major grid style={dotted},
		colorbar,
		colorbar/width=5pt,
		colormap name=mycolormap,
		colorbar style={ylabel={achieved \GFLOPS{}},yticklabel style={font=\tiny,text width=0.7em,}},
		view={0}{90},
	]

	\addplot3[ %
	    scatter=true,
	    only marks,
	    mark=*,
	    color=black,
	    point meta=explicit,
	    visualization depends on = {z/7 \as \perpointmarksize},
	    scatter/@pre marker code/.append style={/tikz/mark size=\perpointmarksize},
	    visualization depends on={meta \as \nodedescription},
	    nodes near coords*={\numprint{\nodedescription}},
		every node near coord/.append style={xshift=0pt,yshift=-16pt,font=\tiny},
	]  table[x=tilesize,y=core_count,z=power8_xl_size_10,meta=power8_xl_10] {./results/power8_autotuning.csv};

	\end{loglogaxis}

\end{tikzpicture}
\end{minipage}
\begin{minipage}{0.495\textwidth}
\centering
\textbf{Single precision, GNU compiler}
\begin{tikzpicture}
	\begin{loglogaxis}[
		width=0.9\textwidth,
		height=0.27\textheight,
		major tick length={1.5pt},
		xlabel={Tile size $T$},
		xtick={16,32,64,128,256,512},
		xticklabels={16,32,64,128,256,512},
		xlabel style={font=\scriptsize},
		xticklabel style={font=\scriptsize},
		ylabel={Hardware threads per core},
		ytick={20,40,80,160},
		yticklabels={1,2,4,8},
		ylabel style={font=\scriptsize},
		yticklabel style={font=\scriptsize},
		zlabel={\GFLOPS},
		grid=major,
		xmin = 10,
		xmax = 850,
		ymin = 13,
		ymax = 250,
		major grid style={dotted},
		colorbar,
		colorbar/width=5pt,
		colormap name=mycolormap,
		colorbar style={ylabel={achieved \GFLOPS{}},yticklabel style={font=\tiny,text width=0.7em,}},
		view={0}{90},
	]

	\addplot3[ %
	    scatter=true,
	    only marks,
	    mark=*,
	    color=black,
	    point meta=explicit,
	    visualization depends on = {z/6.5 \as \perpointmarksize},
	    scatter/@pre marker code/.append style={/tikz/mark size=\perpointmarksize},
	    visualization depends on={meta \as \nodedescription},
	    nodes near coords*={\numprint{\nodedescription}},
		every node near coord/.append style={xshift=0pt,yshift=-16pt,font=\tiny},
	]  table[x=tilesize,y=core_count,z=power8_gcc_float_size_10,meta=power8_gcc_float_10] {./results/power8_autotuning.csv};

	\end{loglogaxis}
\end{tikzpicture}
\end{minipage}
\begin{minipage}{0.495\textwidth}
\centering
\textbf{Double precision, GNU compiler}
\begin{tikzpicture}
	\begin{loglogaxis}[
		width=0.9\textwidth,
		height=0.27\textheight,
		major tick length={1.5pt},
		xlabel={Tile size $T$},
		xtick={16,32,64,128,256,512},
		xticklabels={16,32,64,128,256,512},
		xlabel style={font=\scriptsize},
		xticklabel style={font=\scriptsize},
		ylabel={Hardware threads per core},
		ytick={20,40,80,160},
		yticklabels={1,2,4,8},
		ylabel style={font=\scriptsize},
		yticklabel style={font=\scriptsize},
		zlabel={\GFLOPS},
		grid=major,
		xmin = 10,
		xmax = 850,
		ymin = 13,
		ymax = 250,
		major grid style={dotted},
		colorbar,
		colorbar/width=5pt,
		colormap name=mycolormap,
		colorbar style={ylabel={achieved \GFLOPS{}},yticklabel style={font=\tiny,text width=0.7em,}},
		view={0}{90},
	]

	\addplot3[ %
	    scatter=true,
	    only marks,
	    mark=*,
	    color=black,
	    point meta=explicit,
	    visualization depends on = {z/4.2 \as \perpointmarksize},
	    scatter/@pre marker code/.append style={/tikz/mark size=\perpointmarksize},
	    visualization depends on={meta \as \nodedescription},
	    nodes near coords*={\numprint{\nodedescription}},
		every node near coord/.append style={xshift=0pt,yshift=-16pt,font=\tiny},
	]  table[x=tilesize,y=core_count,z=power8_gcc_size_10,meta=power8_gcc_10] {./results/power8_autotuning.csv};

	\end{loglogaxis}

\end{tikzpicture}
\end{minipage}
	\caption{Achievable \GFLOPS{} for IBM Power8 processor depending on the compiler, the floating point precision, the chosen tile size of the tiled matrix multiplication algorithm and the used hardware threads per core. The bigger the mark size the higher the achieved \GFLOPS{}. The mark radius is calculated with ${(\text{achivied }\GFLOPSinner{})}^{\sfrac{5}{7}}$ as this has been shown a good value for human perception\cite{Gum11}.}
	\label{fig:results_power8}
\end{figure}
